ArtCrafter: Text-Image Aligning Style Transfer via Embedding Reframing

Recent years have witnessed significant advancements in text-guided style transfer, primarily attributed to innovations in diffusion models. These models excel in conditional guidance, utilizing text or images to direct the sampling process. However, despite their capabilities, direct conditional guidance approaches often face challenges in balancing the expressiveness of textual semantics with the diversity of output results while capturing stylistic features. To address these challenges, we introduce ArtCrafter, a novel framework for text-to-image style transfer. Specifically, we introduce an attention-based style extraction module, meticulously engineered to capture the subtle stylistic elements within an image. This module features a multi-layer architecture that leverages the capabilities of perceiver attention mechanisms to integrate fine-grained information. Additionally, we present a novel text-image aligning augmentation component that adeptly balances control over both modalities, enabling the model to efficiently map image and text embeddings into a shared feature space. We achieve this through attention operations that enable smooth information flow between modalities. Lastly, we incorporate an explicit modulation that seamlessly blends multimodal enhanced embeddings with original embeddings through an embedding reframing design, empowering the model to generate diverse outputs. Extensive experiments demonstrate that ArtCrafter yields impressive results in visual stylization, exhibiting exceptional levels of stylistic intensity, controllability, and diversity.

==> Figures/PerceiverAttn.tex <==
\begin{figure}%[t]
\centering
\includegraphics[width= \linewidth]{Images/PerceiverAttn.pdf}
\caption{Visualization results of \shortname architecture trained under different datasets respectively.}
\label{fig:PerceiverAttn}
\end{figure}

==> Figures/pre_N.tex <==
\begin{figure}%[t]
\centering
\includegraphics[width= \linewidth]{Images/pre_N.pdf}
\caption{Visualization results of \shortname architecture trained under different datasets respectively.}
\label{fig:pre_N}
\end{figure}

==> Sections/7_biography.tex <==
%\section{Biography Section}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/huangnisha.png}}]{Nisha Huang} received her B.S. degree in Aeronautical Information Engineering from Beihang University, Beijing, China, in 2021. After that, she obtained her M.S. degree in Artificial Intelligence from the University of Chinese Academy of Sciences, Beijing, China, in 2024. Currently, she is pursuing her PhD in Electronic Information at Tsinghua University. And she is conducting research at the PengCheng Laboratory. Her research interests include generative models, multimedia analysis, and computer vision.

\end{IEEEbiography}

%---------------------------------------- Kaer Huang ----------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/kaer huang.png}}]{Kaer Huang} received the MS degree from North China University, Taiyuan, China. He is currently working at Lenovo Research, Beijing, China. His research interests include perception algorithm, efficient large language models, reinforcement learning for GUI agents.
\end{IEEEbiography}

%---------------------------------------- Yifan Pu ----------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/yifan pu.png}}]{Yifan Pu} received the BS degree in Automation from Beihang University, Beijing, China, in 2020. After that, he was a Master's student with the Department of Automation, Tsinghua University, Beijing, China. He is currently pursuing the PhD degree after transferring into the doctoral program. His research interests include computer vision, machine learning, and deep learning.
\end{IEEEbiography}

%---------------------------------------- Jiangshan Wang ---------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/jiangshan wang.png}}]{Jiangshan Wang} received his B.S degree in Beijing University of Posts and Telecommunications in 2023. He is currently pursuing the M.S. degree in Artificial Intelligence at Tsinghua University. His research interests include computer vision and generative models.
\end{IEEEbiography}

%---------------------------------------- Jie Guo ----------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/jie guo.png}}]{Jie Guo} received her doctoral degree in School of Optics and Photonics from Beijing Institute of Technology in 2021. She is currently an assistant researcher in PengCheng Laboratory. Her main research areas include artificial intelligence, digital humans, virtual reality, and human-computer interaction.
\end{IEEEbiography}

%---------------------------------------- Yiqiang Yan ----------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/yanyiqiang.png}}]{Yiqiang Yan} received the MS degree from Tsinghua University. He is currently the chief researcher of Lenovo, Beijing, China. His research interests include efficient large language models, reinforcement learning for GUI agents.
\end{IEEEbiography}

%---------------------------------------- Xiu Li ----------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography_images/lixiu.jpg}}]{Xiu Li}
(Member, IEEE) received a Ph.D. degree in computer-integrated manufacturing from the Nanjing University of Aeronautics and Astronautics, Nanjing, China, in 2000. From then to 2002, she served as a Post-Doctoral Fellow at the Department of Automation, Tsinghua University, Beijing, China. From 2003 to 2010, she served as an Associate Professor at the Department of Automation, at Tsinghua University. Since 2016, she has been a Full Professor at the Tsinghua Shenzhen International Graduate School, Tsinghua University, Shenzhen, China. Her research interests are in the areas of data mining, deep learning, computer vision, and image processing.
\end{IEEEbiography}


%---------------------------------------- Tong-Yee Lee ----------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{Biography_images/tony_photo1_tvcg.jpg}}]{Tong-Yee Lee} (Senior Member, IEEE) received the Ph.D. degree in computer engineering from Washington State University, Pullman, in May 1995. He is currently a Chair Professor in the Department of Computer Science and Information Engineering, at National Cheng-Kung University, Tainan City, Taiwan. He leads the Computer Graphics Laboratory, National Cheng-Kung University (http://graphics.csie.ncku.edu.tw). His current research interests include computer graphics, non-photorealistic rendering, medical visualization, virtual reality, and media resizing. He is a Senior Member of the IEEE and a Member of the ACM. He also serves on the editorial boards of the IEEE Transactions on Visualization and Computer Graphics.
\end{IEEEbiography}


